Fast simulation of the CEPC detector with Delphes

Fast simulation tools are highly appreciated in particle physics phenomenology studies, especially in the exploration of the physics potential of future experimental facilities. The Circular Electron Positron Collider is a proposed Higgs and Z factory that can precisely measure the Higgs boson properties and the electroweak precision observables. A fast-simulation toolkit dedicated to the CEPC detector has been developed using Delphes. The comparison shows that this fast simulation tool is highly consistent with the full simulation, on a set of benchmark distributions. Therefore, we recommend this fast simulation toolkit for CEPC phenomenological investigations.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = delphes_cpc 

default: testlatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


